Rank-smoothed Pairwise Learning In Perceptual Quality Assessment

Conducting pairwise comparisons is a widely used approach in curating human perceptual preference data. Typically raters are instructed to make their choices according to a specific set of rules that address certain dimensions of image quality and aesthetics. The outcome of this process is a dataset of sampled image pairs with their associated empirical preference probabilities. Training a model on these pairwise preferences is a common deep learning approach. However, optimizing by gradient descent through mini-batch learning means that the "global" ranking of the images is not explicitly taken into account. In other words, each step of the gradient descent relies only on a limited number of pairwise comparisons. In this work, we demonstrate that regularizing the pairwise empirical probabilities with aggregated rankwise probabilities leads to a more reliable training loss. We show that training a deep image quality assessment model with our rank-smoothed loss consistently improves the accuracy of predicting human preferences.

==> Rank Smoothing/definitions.tex <==
\DeclareMathOperator{\sigmoid}{sigmoid}

\newcommand{\Pairs}{\mathcal{P}}
\newcommand{\dom}{\mathcal{X}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\EE}{\mathbb{E}}

\newcommand{\loss}{L(\Theta|\, \Pairs)}
\newcommand{\error}{\text{error}(\alpha, \beta)}

\newcommand{\pl}{p^\text{{\tiny local}}}
\newcommand{\pg}{p^\text{{\tiny global}}}
\newcommand{\pe}{p}

\newcommand{\Cl}{C^\text{{\tiny local}}}
\newcommand{\Cg}{C^\text{{\tiny global}}}


\newcommand{\x}{\bm{x}}

\newcommand{\Pe}{\Pi}
\renewcommand{\P}{\bm{\Pe}}

\newcommand{\se}{\pi}
\newcommand{\s}{\bm{\se}}

\newcommand{\we}{\omega}
\newcommand{\w}{\bm{\we}}
